Application of federated learning techniques for arrhythmia classification using 12-lead ECG signals

Artificial Intelligence-based (AI) analysis of large, curated medical datasets is promising for providing early detection, faster diagnosis, and more effective treatment using low-power Electrocardiography (ECG) monitoring devices information. However, accessing sensitive medical data from diverse sources is highly restricted since improper use, unsafe storage, or data leakage could violate a person's privacy. This work uses a Federated Learning (FL) privacy-preserving methodology to train AI models over heterogeneous sets of high-definition ECG from 12-lead sensor arrays collected from six heterogeneous sources. We evaluated the capacity of the resulting models to achieve equivalent performance compared to state-of-the-art models trained in a Centralized Learning (CL) fashion. Moreover, we assessed the performance of our solution over Independent and Identical distributed (IID) and non-IID federated data. Our methodology involves machine learning techniques based on Deep Neural Networks and Long-Short-Term Memory models. It has a robust data preprocessing pipeline with feature engineering, selection, and data balancing techniques. Our AI models demonstrated comparable performance to models trained using CL, IID, and non-IID approaches. They showcased advantages in reduced complexity and faster training time, making them well-suited for cloud-edge architectures.

==> sec-append.tex <==
% \section{Diagnoses and abbreviations for the selected diagnoses} \label{app_selectedCategories}



% \section{Metrics}  \label{app_metrics}


% \section{Label distribution for the Non-IID method by local node} \label{app_fl_label_distro_filtered_ROS_SMT}

% \section{Label distribution for the filtered dataset by each local node} \label{app_fl_label_distro_filtered}


% \section{Data sources description} \label{app_datasetsSummary}




% \section{Fine-tuning grid for DNN} \label{app_gridDNN}





% \section{Typical ECG waveform} \label{app_ECG_waveform}



% \section{Train and Validation accuracy among local nodes for TEAM2 (the best model)} \label{app_iid_local_nodes_accxx}

% \begin{figure*}[ht]
% \centering
% \includegraphics[width=0.8\textwidth]{paper-images/iid_local_nodes_acc.png}
% \caption{Train and Validation accuracy among local nodes for TEAM2 (the best model)}
% \label{fig:iid_local_nodes_accxx}
% \end{figure*}

% \section{Hardware specification used to train models} \label{app_architecture_config}


% \section{Scenarios tried during modelling phase} \label{app_scenarios_models}




% \section{Feature normalization} \label{app_robustscaler_eq}
% $\mbox{norm}\left({}_{f}x_{i}^{c}\right) = \frac{{}_{f}x_i^c - \bar{{}_{f}x^c}}{{}_{f}x_{q_{75}}^c - {}_{f}x_{q_{25}}^c}$ where $f$ is one of the $636$ features, $\bar{{}_{f}x^c}$ is the median and ${}_{f}x_{q_{35}}^c$ and ${}_{f}x_{q_{75}}^c$ are the 25th and 75th percentiles computed over all the values in the entire federated data set for the given feature $f$ in channel $c$. 

% \begin{equation} \label{robustscaler_eq}
% \mbox{norm}\left({}_{f}x_{i}^{c}\right) = \frac{{}_{f}x_i^c - \bar{{}_{f}x^c}}{{}_{f}x_{q_{75}}^c - {}_{f}x_{q_{25}}^c}
% \end{equation}
%


% \section{DNN architecture} \label{app_DNN_architecture}



